Generative Image Inpainting with Contextual Attention

Recent deep learning based approaches have shown promising results for the challenging task of inpainting large missing regions in an image. These methods can generate visually plausible image structures and textures, but often create distorted structures or blurry textures inconsistent with surrounding areas. This is mainly due to ineffectiveness of convolutional neural networks in explicitly borrowing or copying information from distant spatial locations. On the other hand, traditional texture and patch synthesis approaches are particularly suitable when it needs to borrow textures from the surrounding regions. Motivated by these observations, we propose a new deep generative model-based approach which can not only synthesize novel image structures but also explicitly utilize surrounding image features as references during network training to make better predictions. The model is a feed-forward, fully convolutional neural network which can process images with multiple holes at arbitrary locations and with variable sizes during the test time. Experiments on multiple datasets including faces (CelebA, CelebA-HQ), textures (DTD) and natural images (ImageNet, Places2) demonstrate that our proposed approach generates higher-quality inpainting results than existing ones. Code, demo and models are available at: https://github.com/JiahuiYu/generative_inpainting.

==> algo.tex <==
\section{Improved Generative Inpainting Network}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=1.\linewidth]{fig/framework.png}
\end{center}
   \caption{Illustration of framework.}
\label{fig:framework}
\end{figure*}

In this section, we introduce an improved generative image inpainting network based on work~\cite{iizuka2017globally} as our baseline model. In addition to dilated convolution, global and local GAN proposed in work~\cite{iizuka2017globally}, we propose several enhancements on inpainting network architecture and training objectives. The overview of our improved framework is shown in Figure~\ref{fig:framework}. It is a remarkable fact that the improved model converges faster and stabler. For the Places2~\cite{zhou2017places} dataset, we dramatically reduce training time for convergence from 11,520 GPU-hours (Nvidia K80) to 120 GPU-hours (Nvidia GTX 1080). Moreover, image blending post-processing step in~\cite{iizuka2017globally} is no longer necessary. Thus, we use our improved version as baseline.

\textbf{Inpainting network} As mentioned in~\cite{iizuka2017globally}, receptive field size of output neurons (a.k.a.\ spatial support) is especially important for inpainting large holes. Thus, Iizuka et al.\ \cite{iizuka2017globally} introduce dilated convolution. To further increase receptive field size and stabilize training, we introduce another network which predicts coarse structures and color as roughout results. It is trained with reconstruction loss explicitly and gradients from deeper layers jointly, which can be viewed as a mimic of residual learning~\cite{he2016deep} or deep supervision~\cite{lee2015deeply}. The inpainting network is designed in thin and deep scheme thus has less parameters than work~\cite{iizuka2017globally}.

Moreover, we use symmetric (or reflective) padding for all convolution layers. Batch normalization layers~\cite{ioffe2015batch} are removed. ELUs~\cite{clevert2015fast} are used as activation function. We clip the value from output layer instead of using \(tanh\) or \(sigmoid\) function. Furthermore, we separate the global and local GAN instead of concatenate features after fully-connected layer. More details can be found in supplementary.

\textbf{Global and local Wasserstein GAN} We introduce two Wasserstein GAN critics for modeling global and local content consistency: a local one on generated bounding box region and a global one on entire completed image. Different from previous generative inpainting networks~\cite{iizuka2017globally, li2017generative, pathak2016context}, where authors use DCGAN~\cite{radford2015unsupervised} for adversarial supervision, we formulize improved WGAN~\cite{arjovsky2017wasserstein, gulrajani2017improved} with modification on gradient penalty term for image inpainting.

To review, WGAN uses \textit{Earth-Mover} distance (a.k.a.\ \textit{Wasserstein-1}) distance \(W(\mathbb{P}_r, \mathbb{P}_g)\) instead of \textit{Total Variation}, \textit{Kullback-Leibler} or \textit{Jensen-Shannon} divergence for measure of two distributions. The objective function for a WGAN is constructed by applying the \textit{Kantorovich-Rubinstein} duality to obtain:
\[ \min_G\max_{D \in \mathcal{D}} E_{\mathbf{x} \sim \mathbb{P}_r}[D(\mathbf{x})] - E_{\tilde{\mathbf{x}} \sim \mathbb{P}_g}[D(\tilde{\mathbf{x}})],\]
where \(\mathcal{D}\) is the set of 1-Lipschitz functions and \(\mathbb{P}_g\) is the model distribution implicitly defined by \(\tilde{\mathbf{x}} = G(\mathbf{z})\). \(\mathbf{z}\) is the input to generator which can be a vector of random noise from uniform distribution or samples from a set.

To enforce the Lipschitz constraint on the critic, Arjovsky et al.~\cite{arjovsky2017wasserstein} proposed to clip the weights of the critic to lie within a compact space \([-c, c]\), where \(c\) is a constant value. Gulrajani et al.~\cite{gulrajani2017improved} proposed an improved version with a gradient penalty term
\[\lambda E_{\hat{\mathbf{x}} \sim \mathbb{P}_{\hat{\mathbf{x}}}}(\lVert \nabla_{\hat{\mathbf{x}}} D(\hat{\mathbf{x}})\rVert_2 - 1)^2,\]
where \(\mathbf{\hat x}\) is sampled from straight lines between points sampled from distribution \(\mathbb{P}_g\) and \(\mathbb{P}_r\). The reason is that the gradient of \(D^*\) at all points \(\hat{\mathbf{x}} = (1 - t)\mathbf{x} + t\tilde{\mathbf{x}}\) on the straight line should points directly towards current sampled \(\tilde{\mathbf{x}}\), meaning \(\nabla_{\mathbf{\hat x}} D^*(\hat{\mathbf{x}}) = \frac{\tilde{\mathbf{x}}-\hat{\mathbf{x}}}{\lVert \tilde{\mathbf{x}}-\hat{\mathbf{x}}\rVert}\). For image inpainting, we only try to predict hole regions thus the gradient penalty should be directly applied only on pixels in holes, not in the conditional inputs (surrounding pixels). This can be implemented with multiplication of gradients and input mask as follows:
\[\lambda E_{\hat{\mathbf{x}} \sim \mathbb{P}_{\hat{\mathbf{x}}}}(\lVert \nabla_{\hat{\mathbf{x}}} D(\hat{\mathbf{x}}) \odot (\mathbf{1} - \mathbf{m})\rVert_2 - 1)^2,\]
assuming \(m_{i,j} = 0\) means the missing pixel and \(1\) otherwise. \(\lambda\) is set to 10 in all experiments.

We use a weighted sum of pixel-wise \(\ell_1\) loss (instead of mean-square-error in~\cite{iizuka2017globally}) and WGAN adversarial losses. Note that in primal space, \textit{Wasserstein-1} distance in WGAN is based on \(\ell_1\) ground distance:
\[ W(\mathbb{P}_r, \mathbb{P}_g) = \inf_{\gamma \in \prod(\mathbb{P}_r, \mathbb{P}_g)} E_{(\mathbf{x},\mathbf{y}) \sim \gamma}[\lVert \mathbf{x} - \mathbf{y} \rVert],\]
where \(\prod(\mathbb{P}_r, \mathbb{P}_g)\) denotes the set of all joint distributions \(\gamma(\mathbf{x}, \mathbf{y})\) whose marginals are respectively \(\mathbb{P}_r\) and \(\mathbb{P}_g\). Intuitively, the pixel-wise reconstruction loss directly regresses holes to the current ground truth image, while WGANs implicitly learn potentially correct images and train generator with adversarial gradients. Both losses measure distance of images with pixel-wise \(\ell_1\) difference.

\textbf{Spatially discounted reconstruction loss}
To fill the hole in an image, there could exist many plausible solutions. Intuitively, pixels near hole boundaries have less label variations than ones in center of hole. In other words, if all pixels are treated equally with reconstruction loss, the convolutional filters are trained to focus on predicting the hard-to-guess hole center, thus deteriorating boundary consistency.

The same problem is also experienced in reinforcement learning. When long term rewards have large variations during sampling, people use temporal discounted rewards over sampled trajectories~\cite{sutton1998reinforcement}. Similarly, we introduce spatially discounted reconstruction loss using a simple pre-computed loss weighting mask \(\mathbf{M}\) controlled by one scalar parameter \(\gamma\). For each pixel in hole, the loss weighting value is computed as \(\gamma^{l}\), where \(l\) is the distance to the nearest rectangle boundary. \(\gamma\) is set to 0.99 in all experiments.

The problem is also addressed in~\cite{pathak2016context, yeh2016semantic}. Importance weighted context loss, proposed in~\cite{yeh2016semantic}, is pixel-wise loss spatially weighted by ratio of uncorrupted pixels within fixed windows size (\(7 \times 7\) pixels). Pathak et al.\ \cite{pathak2016context} predict a slightly larger patch with higher loss weighting (\(\times 10\)) in overlapped region (7 pixels). For inpainting large holes, the proposed discounted loss makes more sense and introduces almost zero computational overhead. Experiments show that it slightly improves visual quality. We use discounted \(\ell_1\) reconstruction loss as default.

%\textbf{Symmetric padding} Padding pixels is required for convolution to keep output dimension the same as input dimension (e.g. padding one pixel on each side for three by three convolutional kernel). For image recognition models, people usually pad zero values. We use symmetric padding in all convolution layers in inpainting network. Symmetric (or reflective) padding has two benefits: 1) It results in better color coherence for testing an image of resolution different from training images. 2) It enables our framework to fill holes on image borders with less artifacts. An alternative approach is to use another channel as input to indicate the image borders and use varied image resolutions during training.

\section{Proposed Algorithm}

\subsection{Contextual attention} \label{subsec:attention}

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1.\linewidth]{fig/contextual_attention_layer.png}
    \end{center}
    \caption{Contextual attention layer.}
    \label{fig:contextual_attention_layer}
\end{figure}

Convolution neural networks take local features layer-by-layer thus is not effective for borrowing patches of interest, especially the ones at distant spatial locations. To solve the problem, we consider attention mechanism in deep models. We find existing feed-forward spatial attention modules are very limited on the task of image inpainting. Thus, we propose a novel feed-forward contextual attention layer that can be trained in an end-to-end manner.

In short, contextual attention layer is designed with convolution for matching, softmax for comparison and deconvolution for pasting. We also introduce two additional convolutions to propagate attention scores horizontally and vertically which encourage to attend on coherent regions instead of individual pixels. Moreover, we introduce several choices to improve memory efficiency with almost no drop of performance. Finally, it is noteworthy that contextual attention layer can take images of arbitrary resolution during testing.

\textbf{Match and paste}
We consider the problem where we have features of missing pixels (foreground) and surroundings (background). As shown in Figure~\ref{fig:contextual_attention_layer}, we firstly extract patches (\(3 \times 3\)) located in backgrounds and reshape them as convolutional filters. To match missing patches \(\{f_{(x, y)}\}\) with surrounding patches \(\{b_{x',y'}\}\), we use normalized inner product (cosine similarity)
\[s_{x,y,x',y'} = \langle \frac{f_{x,y}}{||f_{x,y}||}, \frac{b_{x',y'}}{||b_{x',y'}||}\rangle,\]
where \(s_{x,y,x',y'}\) is the matching score of center patch located in background \((x',y')\) and foreground patch located in \((x, y)\). We then normalize the matching score with scaled softmax along \(x'y'\)-dimension to get attention score \(s^*_{x,y,x',y'} = \textit{softmax}_{x',y'} (\lambda s_{x,y,x',y'})\), where \(\lambda\) is a constant value. This can be efficiently implemented as convolution and channel-wise softmax as shown in Figure~\ref{fig:contextual_attention_layer}. Similarly, as the final step, we reuse extracted patches \(\{b_{x',y'}\}\) as deconvolutional filters for differentiable patch pasting. Values of overlapped pixels are averaged.

We notice that previously several works~\cite{chen2016fast, li2016combining} utilize convolution to speed up computing nearest neighbor fields for style transfer tasks. Differently, those methods directly get a result with the maximum score, remaining the whole module non-differentiable. We should also notice that contextual attention layer can be viewed as a kind of soft PatchMatch~\cite{barnes2009patchmatch} on feature space learned with deep neural networks.

\textbf{Attention propagation}
We further introduce coherency prior in contextual attention layer which significantly improves inpainting quality. The idea of coherency prior is that a shifted foreground patch is likely corresponding to an equal shift in the background patch by the natural of image data. That is, for example, \(s^*_{x, y, x', y'}\) usually have very close value with \(s^*_{x+1, y, x'+1, y'}\). To encourage resulted attention map consists of coherence patches instead of individual pixels, we perform a left-right propagation followed by a top-down propagation with kernel size of k. That is:
\[
    \begin{split}
        {s^h}_{x, y, x', y'} = & \sum_{i \in \{-k, ..., k\}}s^*_{x+i, y, x'+i, y'}, \\ {s^v}_{x, y, x', y'} = & \sum_{j \in \{-k, ..., k\}}s^h_{x, y+j, x', y'+j}.
    \end{split}
\]
The propagation can be efficiently implemented as convolution with fixed constant kernel (i.e.\ identity matrix) and proper corner paddings. k is set to 2 in all of our experiments. This property can significantly improves inpainting results in the forward path and provides richer gradients in the backward path. Note that it is also possible to learn a spatial propagation with a few convolutions and activations. With attention propagation, the resulted attention map is often formed from coherent regions.

\textbf{Memory efficiency}
Assume that we have a feature of resolution \(128 \times 128\) with missing region of resolution \(64 \times 64\). Then the resulted number of convolutional filters is 12,288. This may cause too much memory overhead for GPUs. To overcome the issue, we introduce two options: 1) Extracting background patches with strides to reduce the number of filters. 2) Reducing resolution of foreground attention map for convolution and then use background patches of raw resolution to paste with strides.

\subsection{Unified inpainting network} \label{subsec:unified}

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1.\linewidth]{fig/unified_attention_network.png}
    \end{center}
    \caption{Unified with attention.}
    \label{fig:unified_attention}
\end{figure}

To borrow background patches without lossing ability of hallucinating novel contents, we introduce two parallel encoders as shown in Figure~\ref{fig:unified_attention} based on Figure~\ref{fig:framework}. The bottom encoder specifically focuses on hallucinating contents with layer-by-layer (dilated) convolution, while the top one tries to attend on background features of interest. Output features from two encoders are then aggregated and fed into single decoder to obtain the final output.

For training, given a \textit{raw image} \(\mathbf{x}\) of size \(H \times W\), we sample a boolean \textit{image mask} \(\mathbf{m}\) on a random location. \textit{Input image} \(\mathbf{z}\) is corrupted from \textit{raw image} as \(\mathbf{z} = \mathbf{x} \odot \mathbf{m}\). Inpainting network \(G\) takes channel-wise concatenation of \textit{input image} and \textit{image mask} as input, and output \textit{predicted image} \(\mathbf{x'} = G(\mathbf{z, m})\) with size the same as input (i.e.\ \(H \times W\)). Pasting the masked region of \(\mathbf{x'}\) to \textit{input image}, we get \textit{completed image} \(\tilde{\mathbf{x}} = \mathbf{z} + \mathbf{x'} \odot \mathbf{(1-m)}\). Image values are linearly scaled from range \([0, 256]\) to \([-1, 1]\) in all experiments.

To sample \textit{image mask} with variable size, we firstly sample a mask \(\mathbf{m'}\) with size exactly as \(h \times w\) on random location. Then we sample another mask \(\mathbf{m}\) inside \(\mathbf{m'}\) with random height in range \([\frac{3}{4}h, h]\) and width in \([\frac{3}{4}w, w]\) on a random location as final \textit{image mask}. Note that the input to local GAN has to be with fixed size because of final fully-connected layers. Thus,  we take the bounding box cropping of \textit{completed image} \(\tilde{\mathbf{x}}\) by mask \(\mathbf{m'}\) as input to local GAN, and use \textit{completed image} \(\tilde{\mathbf{x}}\) as input to global GAN. Note that unlike work~\cite{iizuka2017globally}, we do not sample another random mask to construct real data for local GAN, instead we use same mask \(\mathbf{m'}\) to crop ground truth image as real data. We describe training procedure in algorithm~\ref{algo:algo}.

\input{tex_figures/algo.tex}


==> tex_figures/no_l1_figure.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.145\textwidth]{fig/no_l1/case10_raw.png}
\includegraphics[width=0.145\textwidth]{fig/no_l1/case10_incomplete.png}
\includegraphics[width=0.145\textwidth]{fig/no_l1/case10_complete.png}

\includegraphics[width=0.145\textwidth]{fig/no_l1/case8_raw.png}
\includegraphics[width=0.145\textwidth]{fig/no_l1/case8_incomplete.png}
\includegraphics[width=0.145\textwidth]{fig/no_l1/case8_complete.png}

\includegraphics[width=0.145\textwidth]{fig/no_l1/case27_raw.png}
\includegraphics[width=0.145\textwidth]{fig/no_l1/case27_incomplete.png}
\includegraphics[width=0.145\textwidth]{fig/no_l1/case27_complete.png}

\caption{Without $\ell_1$ loss, inpainting network is not able to capture global contents and easily hallucinates meaningless structures. Also, there is obvious boundary incoherence.}
\label{fig:expr_no_l1}
\end{figure}

==> tex_figures/param.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c c c c c}
\hline
Method & trainable parameter size & inpainting network size\\
\hline
\cite{iizuka2017globally} & 32M & 5.8M\\
Ours & \textbf{10M} & \textbf{2.9M}\\
\hline
\end{tabular}
\end{center}
\caption{Results. Ours is better.}
\label{tab:param}
\end{table}

==> tex_figures/speed.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c c c c c}
\hline
Method & \(256 \times 256\) & \(512 \times 512\) & \(1024 \times 1024\)\\
\hline
\cite{iizuka2017globally} (CPU) & \textbf{0.3s} & \textbf{1.2s} & \textbf{4.0s} & \\
Ours (CPU) & 0.4s & 1.5s & 18.2s\\
\cite{iizuka2017globally} (GPU) & \textbf{0.1s} & \textbf{0.1s} & \textbf{0.5s}\\
Ours (GPU) & 0.1s & 0.2s & 1.1s\\
\hline
\end{tabular}
\end{center}
\caption{Results. Ours is inferior.}
\label{tab:speed}
\end{table}
